Optimal Network Topology of Multi-Agent Systems subject to Computation and Communication Latency (with proofs)

We study minimum-variance feedback-control design for a networked control system with retarded dynamics, where inter-agent communication is subject to latency. We prove that such a design can be solved efficiently for circular formations and compute near-optimal control gains in closed form. We show that the centralized control architecture is in general suboptimal when the communication increase with the number of links, and propose a control-driven optimization of the network topology.

==> Sections/numerical-simulations.tex <==
%!TEX ROOT = ../centralized_vs_distributed.tex

\section{Numerical simulations}\label{sec:simulations}

%To validate the theoretical results, 
To assess the behavior of the proposed control,
we have simulated system~\eqref{eq:stateErrorDynamics} in Simulink with 
size $ N = 50 $ agents,
minimum delay $ \tau_{\textit{min}} = 10\si{\milli\second} $,
sample time $ T_s = 1\si{\milli\second}$, and
differential of the Brownian noise approximated by
a Gaussian process with power $ T_s $.
Also, a linear rate $ f(n) $ was used.
%and linear increase rate of $ \taun $.
The simulations have been performed with initial condition $ \x{}{t} = x_0\delta(t) $ for $ t \in [-\taun, 0] $,
where $ x_0 $ has been sampled from a standard $ N $-dimensional Gaussian distribution
and $ \delta(t) $ is the Kronecker delta. % is drawn according to a standard $ N $-dimensional Gaussian distribution,
Each simulation was averaged over 20 Monte Carlo iterations with the same initial condition.

\begin{figure}
	\centering
	\begin{minipage}[l]{.48\linewidth}
		\includegraphics[width=\linewidth]{sim-n-2-trans}
		\caption{Transient signal ($ n = 2 $).}
		\label{fig:sim-n-2-trans}
	\end{minipage}%
	\hfill
	\begin{minipage}[r]{.48\linewidth}
		\includegraphics[width=\linewidth]{sim-n-10-trans}
		\caption{Transient signal ($ n = 10 $).}
		\label{fig:sim-n-10-trans}
	\end{minipage}
\end{figure}
\begin{figure}
	\centering	
	\begin{minipage}[l]{.48\linewidth}
		\includegraphics[width=\linewidth]{sim-n-2-ss}
		\caption{Steady-state signal with variance $ \sigma_{\textit{ss}}^2(x) \approx 0.08 $ ($ n = 2 $).}
		\label{fig:sim-n-2-ss}
	\end{minipage}%
	\hfill
	\begin{minipage}[r]{.48\linewidth}
		\includegraphics[width=\linewidth]{sim-n-10-ss}
		\caption{Steady-state signal with variance $ \sigma_{\textit{ss}}^2(x) \approx 0.19 $ ($ n = 10 $).}
		\label{fig:sim-n-10-ss}
	\end{minipage}
\end{figure}

~\autoref{fig:sim-n-2-trans}--\ref{fig:sim-n-10-trans} show the converging phase of the signal 
with $ n = 2 $ and $ \taun = 20\si{\milli\second} $ and
with $ n = 10 $ and $ \taun = 100\si{\milli\second} $, respectively.
While the convergence looks slower in the first case,
there are longer oscillations in the second case before $ t = 0.5\si{\second} $.
~\autoref{fig:sim-n-2-ss}--\ref{fig:sim-n-10-ss} show the steady-state signal coordinates
oscillating about the mean of $ x_0 $ which equals approximately $ 0.284 $.
The signal shows bigger oscillations with $ n = 10 $,
the scalar variance $ \sigma_{\textit{ss}}^2 $ being considerably larger than with $ n = 2 $.



==> Sections/optimization-a-max.tex <==
%!TEX ROOT = ../centralized_vs_distributed.tex

\subsubsection{Single gain, maximum variance}
We now focus on optimizing the worst-performing eigenvalue-driven subsystem.
\begin{prob}\label{prob-a-max}
	Given a platoon with $ N $ vehicles, where each vehicle receives measurements from its closest $ n $ neighbors ahead and $ n $ behind, 
	with delay $ \taun $, design the feedback gain $ \alpha $ minimizing the variance of the eigenvalue-driven subsystem~\eqref{eq:scalar-subs-eigs} with maximum variance:
	\begin{equation}\label{eq:problem-a-max}
		\begin{aligned}
			\alpha^*_M &= \argmin_{\alpha\in\Real{}}\;\max\left\lbrace\sigma^2_{\textit{ss}}(\lambda_i)\right\rbrace_{i=1}^N\\
			\mbox{s.t. } & \lambda_i \in\setss(n), \ i = 2,...,N
		\end{aligned}
	\end{equation}
	where $ \lambda_i = \lambda_i(\alpha) $ is the $ i $-th eigenvalue of $ K $.
\end{prob}

\myParagraph{Solution}
In virtue of convexity of $ \sigma^2_{\textit{ss}}(\lambda) $, this problem can be recast as follows:
\begin{equation}\label{eq:problem-a-max-simplified}
	\begin{aligned}
		\alpha^*_M &= \argmin_{\alpha\in\Real{}}\;\max\left\lbrace\sigma^2_{\textit{ss}}(\lambda_m),\sigma^2_{\textit{ss}}(\lambda_M)\right\rbrace\\
		\mbox{s.t. } & \lambda_m,\lambda_M \in\setss(n)
	\end{aligned}
\end{equation}
where $ \lambda_m $ and $ \lambda_M $ are the minimum and maximum nonzero eigenvalues of $ K $, respectively.
Because $ \sigma^2_{\textit{ss}}(\lambda) $ is continuous, and all eigenvalues are increasing with $ \alpha $,
the optimum gain $ \alpha^*_M $ is given by the unique solution of the equation
\begin{equation}\label{eq:a-max-eq-solution}
	\sigma^2_{\textit{ss}}(\alpha f_m) = \sigma^2_{\textit{ss}}(\alpha f_M), \qquad \alpha\in\setss(nf_M)
\end{equation}
where $ \lambda_i = \alpha f_i $ and $ f_m = \min f_i $, $ f_M = \max f_i $, with
\begin{equation}\label{eq:eigCoefficients}
		f_i = 2\left(n-\sum_{j=1}^{n}\cos\left(\dfrac{2\pi (i-1)j}{N}\right)\right), \ i = 2,...,N
\end{equation}
which can be easily solved, \eg with bisection.

\begin{rem}
    Both~\cref{prob-a-sum}--\ref{prob-a-max} can be solved numerically also for band-diagonal feedback matrix $ K $. %, by replacing $ f_i $ with the eigenvalues of $ K(1)$.
\end{rem}

==> Sections/optimization-k-max.tex <==
%!TEX ROOT = ../centralized_vs_distributed.tex

\subsubsection{Symmetric gains, maximum variance}
We now focus on optimizing the worst-performing eigenvalue-driven subsystem with symmetric gains.
\begin{prob}\label{prob-k-max}
	Given a platoon with $ N $ vehicles, where each vehicle receives measurements from its closest $ n $ neighbors ahead and $ n $ behind, 
	and with single-hop communication delay $ \tau $, design the feedback gain $ k_i $, $ i=1,...,n $, minimizing the variance of the eigenvalue-driven subsystem~\eqref{eq:scalar-subs-eigs} with maximum variance:
	\begin{equation}\label{eq:problem-k-max}
		\begin{aligned}
			k^*_M &= \argmin_{k\in\Real{n}}\;\max\left\lbrace\sigma^2_{\textit{ss}}(\lambda_i)\right\rbrace_{i=1}^N\\
			\mbox{s.t. } & \lambda_i \in\setss(n), \ i = 2,...,N
		\end{aligned}
	\end{equation}
	where $ \lambda_i = \lambda_i(k) $ is the $ i $-th eigenvalue of $ K $ and
	$ k = \begin{bmatrix} k_1 & \dots & k_n \end{bmatrix} $.
\end{prob}

\myParagraph{Solution}
Again, we can focus on the following optimization:
\begin{equation}\label{eq:problem-k-max-simplified}
	\begin{aligned}
		k^*_M &= \argmin_{k\in\Real{n}}\;\max\left\lbrace\sigma^2_{\textit{ss}}(\lambda_m),\sigma^2_{\textit{ss}}(\lambda_M)\right\rbrace\\
		\mbox{s.t. } & \lambda_m,\lambda_M \in\setss(n)
	\end{aligned}
\end{equation}
%The above problem is solved in two steps: 
First, the maximum eigenvalue is minimized, constrained to a lower bound for the nonzero minimum eigenvalue:
\begin{equation}\label{eq:problem-k-max-minimize-lambda-max}
	\begin{aligned}
	\tilde{k}_M^* &= \argmin_{k\in\Real{n}} \; \lambda_M(k)\\
		\mbox{s.t. } & \lambda_m(k) \ge 1
	\end{aligned}
\end{equation}
Problem~\eqref{eq:problem-k-max-minimize-lambda-max} is solved when $ \lambda_m = 1 $.
The found eigenvalues, and therefore the feedback gains $ \tilde{k}_{i,M}^* $ solving~\eqref{eq:problem-k-max-minimize-lambda-max},
are now optimal up to a scaling coefficient $\beta$,
which can be retrieved by solving eq.~\ref{eq:a-max-eq-solution} with the corresponding eigenvalue coefficients:
\begin{equation}\label{eq:beta-max-eq-solution}
	\sigma^2_{\textit{ss}}(\beta) = \sigma^2_{\textit{ss}}(\beta\tilde{\lambda}_M^*), \qquad \beta\in \setss(n\tilde{\lambda}_M^*)
\end{equation}
where $ \tilde{\lambda}_M^* $ is the unique optimum of~\eqref{eq:problem-k-max-minimize-lambda-max}.
%The optimal eigenvalues are $ \lambda_m^* = \beta^* $ and $ \lambda_M^* = \beta^*\tilde{\lambda}_M^* $,
%where $ \beta^* $ is the solution of~\eqref{eq:beta-max-eq-solution},
The optimal feedback gains are then computed as $ {k}_{M}^* = \beta^*\tilde{k}_{M}^* $.

\autoref{fig:allmaxvarteo} shows the maximum of the variances $ \sigma^2_{\textit{ss}}(\lambda_i) $
obtained by solving Problems~\ref{prob-a-sum} (blue circles),~\ref{prob-a-max} (red squares) and~\ref{prob-k-max} (yellow triangles),
% for the eigenvalue-driven scalar subsystems~\eqref{eq:scalar-subs-eigs},
with fixed platoon size $ N $ and varying feedback neighborhood size $ n $.
%A trade-off over $ n $ %, representing the feedback effort, 
%can be clearly seen for all three optimizations.
\begin{figure}
	\centering
	\includegraphics[width=0.8\linewidth]{all_max_var_theo}
	\caption{Maximum variance of eigenvalue-driven subsystems $ \max_i{\sigma^{2}_{\textit{ss}}(\lambda_i)} $, $ \lambda_i \neq 0 $ (theoretical).
	(\textbf{Warning:} ignore $ y $-axis label)}
	\label{fig:allmaxvarteo}
\end{figure}



==> Sections/optimization.tex <==
%!TEX ROOT = ../centralized_vs_distributed.tex

\subsection{optimization of feedback gains}
We would like to design the parameters of the feedback matrix $ K $ such that the subsystems~\eqref{eq:scalar-subs-eigs} have solutions as close as possible to the optimal one,
which corresponds to having eq.~\eqref{eq:scalar-subs-eigs} driven by $ \opteig $, with corresponding steady-state variance $ \optvar $.
The latter also corresponds to the power of the deterministic system, according to~\eqref{eq:steady-state-variance},
affecting the settling time of each subsystem~\eqref{eq:scalar-subs-eigs}.\\
We study the following four optimization problems.


